Intuitive and Efficient Roof Modeling for Reconstruction and Synthesis

We propose a novel and flexible roof modeling approach that can be used for constructing planar 3D polygon roof meshes. Our method uses a graph structure to encode roof topology and enforces the roof validity by optimizing a simple but effective planarity metric we propose. This approach is significantly more efficient than using general purpose 3D modeling tools such as 3ds Max or SketchUp, and more powerful and expressive than specialized tools such as the straight skeleton. Our optimization-based formulation is also flexible and can accommodate different styles and user preferences for roof modeling. We showcase two applications. The first application is an interactive roof editing framework that can be used for roof design or roof reconstruction from aerial images. We highlight the efficiency and generality of our approach by constructing a mesh-image paired dataset consisting of 2539 roofs. Our second application is a generative model to synthesize new roof meshes from scratch. We use our novel dataset to combine machine learning and our roof optimization techniques, by using transformers and graph convolutional networks to model roof topology, and our roof optimization methods to enforce the planarity constraint.

==> figures_tex/figtex_ablation_planarity.tex <==
\begin{overpic}[trim=0.5cm 0cm 0cm 0cm,clip,width=1\linewidth,grid=false]{ablation_planarity.pdf}
\put(30,0){\footnotesize \# iter}
\put(20,52){\footnotesize Different Planarity Energy}
\put(-2,7){\footnotesize{\rotatebox{90}{log-scale}}}
\put(-2,30){\footnotesize{\rotatebox{90}{linear-scale}}}

\put(68,44){\footnotesize $E_{\text{Ours}}$}
\put(90,44){\footnotesize $E_{\text{det}}$}
\put(68,20){\footnotesize $E_{\text{proj}}$}
\put(90,20){\footnotesize $E_{\text{cross}}$}

\put(10.5,9){\tiny $t=0.14s$}
\put(25,10){\tiny $t=0.16s$}
\put(36,18){\tiny $t=1.19s$}
\put(50,22){\tiny $t=1.69s$}
\end{overpic}

==> figures_tex/figtex_different_weight.tex <==
\begin{overpic}[trim=0.5cm 0cm 0cm 0cm,clip,width=1\linewidth,grid=false]{different_weights}
    \put(2,35.5){\footnotesize Initialization}
    \put(25,37){\footnotesize $\lambda_1=1$}
    \put(22,34){\footnotesize $\lambda_2=\lambda_3=0$}
    \put(41,37){\footnotesize $\lambda_1=\lambda_2=1$}
    \put(44.5,34){\footnotesize $\lambda_3 = 0$}
    \put(60,37){\footnotesize $\lambda_1 = \lambda_3 = 1$}
    \put(63.5,34){\footnotesize $\lambda_2=0$}
    \put(79,35.5){\footnotesize $\lambda_1=\lambda_2=\lambda_3=1$}
\end{overpic}

==> figures_tex/figtex_heuristics.tex <==
\begin{overpic}[trim=1.2cm 1cm 1.2cm 0cm,clip,width=0.9\linewidth,grid=false]{heuristics}
    \put(14,14.5){\tiny $d_1$}
    \put(22.5,14.5){\tiny $d_2$}
    \put(11,24){\footnotesize $d_1 \approx d_2$}
    
    \put(42.5,0){\tiny $\alpha_1$}
    \put(55,0){\tiny $\alpha_2$}
    \put(45,24){\footnotesize $\alpha_1 \approx \alpha_2$}
    \put(70,12){\tiny $\beta_1$}
    \put(81,12){\tiny $\beta_2$}
    \put(77,24){\footnotesize $\beta_1 + \beta_2 \approx 180^{\circ}$}
    \put(0.8,2){\footnotesize\bfseries (a)}
    \put(36.2,2){\footnotesize\bfseries (b)}
    \put(71,2){\footnotesize\bfseries (c)}
\end{overpic}

==> figures_tex/figtex_planarity_diff_height.tex <==
\begin{overpic}[trim=0cm 0cm 0cm 0cm,clip,width=1\linewidth,grid=false]{planarity_diff_height}
    \put(15,-1){\footnotesize{\# iteration ($k$)}}
    \put(8,38){\footnotesize{Planarity Error (different $h$)}}
    \put(48,30){\scriptsize $h=10$}
    \put(62,30){\scriptsize $h=20$}
    \put(76,30){\scriptsize $h=30$}
    \put(90,30){\scriptsize $h=40$}
    \put(48,17){\scriptsize $h=50$}
    \put(62,17){\scriptsize $h=75$}
    \put(75,17){\scriptsize $h=100$}
    \put(89.5,17){\scriptsize $h=125$}
    \put(48,-1){\scriptsize $h=150$}
    \put(61,-1){\scriptsize $h=200$}
    \put(75,-1){\scriptsize $h=250$}
    \put(89.5,-1){\scriptsize $h=300$}
    
    \put(-2,7){\footnotesize{\rotatebox{90}{log-scale}}}
    \put(-2,22){\footnotesize{\rotatebox{90}{linear-scale}}}
\end{overpic}

==> figures_tex/figtex_vtx_transformer.tex <==
\begin{overpic}[trim=0cm 0cm 0cm 0cm,clip,width=1\linewidth,grid=false]{vtx_transformer.pdf}
    \put(2,14){\tiny $v=(0.4,0.1,0.6)$}
    \put(2,7.5){\tiny $v=(0.1,0.2,0.3)$}
    \put(37.5,17.5){\tiny $\nu_1=0.4$}
    \put(37.5,14.2){\tiny $\nu_2=0.1$}
    \put(37.5,10.9){\tiny $\nu_3=0.6$}
    \put(37.5,7.6){\tiny $\nu_4=0.1$}
    \put(37.5,4.3){\tiny $\nu_5=0.2$}
    
    
    \put(87,20.8){\tiny $p(\nu_1)$}
    \put(87,17.5){\tiny $p(\nu_2\,\vert\, \nu_1)$}
    \put(87,14.2){\tiny $p(\nu_3\,\vert\,\nu_{<3})$}
    \put(87,10.9){\tiny $p(\nu_4\,\vert\,\nu_{<4})$}
    \put(87,7.6){\tiny $p(\nu_5\,\vert\,\nu_{<5})$}
    \put(87,4.3){\tiny $p(\nu_6\,\vert\,\nu_{<6})$}
    
    \put(24.5,10.5){\footnotesize Flatten}
    
    \put(7,26.5){\footnotesize Vertices}
    \put(37,28){\footnotesize Vertex}
    \put(33.5,25){\footnotesize Coordinates}
    \put(55.5,26.5){\footnotesize Vertex Transformer}
    \put(86,28){\footnotesize Prediction}
    \put(84.5,25){\footnotesize Probabilities}
\end{overpic}

==> tables/tb_res_img_reconstruction_old.tex <==
\footnotesize
{\def\arraystretch{1.2}\tabcolsep=0.2em
\begin{tabular}{ccccccccccccccccc}
\toprule[1pt]
\rowcolor{mytbcol!20}
No.   & 1    & 2    & 3    & 4    & 5    & 6    & 7    & 8    & 9    & 10   & 11   & 12   & 13   & 14   & 15   & 16   \\
$n_v$ & 22   & 24   & 25   & 25   & 27   & 27   & 32   & 33   & 33   & 33   & 34   & 35   & 36   & 39   & 39   & 51   \\\rowcolor{mytbcol!20}
$n_f$ & 12   & 17   & 14   & 14   & 15   & 16   & 17   & 20   & 18   & 20   & 18   & 21   & 19   & 22   & 21   & 38   \\\hline
$\text{e}_\text{\textbf{ours}}$ & 0 & 0 & 0 & 0 & 0 & 0  & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0\\\rowcolor{mytbcol!20}
$\text{e}_\text{wss}$ & 0 & 2 & 0 & 0 & 1 & 2  & 1 & 1 & 0 & 2 & 2 & 2 & 1 & 2 & 2 & 2\\\hline 
$t_v$ & 27.6 & 36.6 & 39.3 & 29.4 & 31.4 & 25.5 & 43.9 & 40.8 & 43.5 & 49.8 & 49.9 & 52.5 & 50.9 & 55.5 & 58.3 & 66.6 \\\rowcolor{mytbcol!20}
$t_f$ & 61.4 & 77.7 & 112  & 67.9 & 82.2 & 66.5 & 106  & 102  & 109  & 116  & 97.3 & 104  & 126  & 143  & 118  & 214  \\
$t_o$ & 0.42 & 1.20 & 0.73 & 0.55 & 0.61 & 0.89 & 0.94 & 2.23 & 1.47 & 1.05 & 0.72 & 1.58 & 1.24 & 1.34 & 2.52 & 3.59 \\\rowcolor{mytbcol!20}
$t_{\text{\textbf{ours}}}$  & 89.4 & 115 & 153 & 97.9 & 114 & 92.9 & 151 & 145 & 155 & 167 & 148 & 158 & 179 & 199 & 178 & 284 \\
$t_{\text{wss}}$ & - & 300 & - & - & 60 & 180 & 180 & 300 & - & 120 & 180 & 60 & 60 & 480 & 180 & 360\\
\bottomrule[1pt]
\end{tabular}
}
